Data Guards: Challenges and Solutions for Fostering Trust in Data

From dirty data to intentional deception, there are many threats to the validity of data-driven decisions. Making use of data, especially new or unfamiliar data, therefore requires a degree of trust or verification. How is this trust established? In this paper, we present the results of a series of interviews with both producers and consumers of data artifacts (outputs of data ecosystems like spreadsheets, charts, and dashboards) aimed at understanding strategies and obstacles to building trust in data. We find a recurring need, but lack of existing standards, for data validation and verification, especially among data consumers. We therefore propose a set of data guards: methods and tools for fostering trust in data artifacts.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/_03.5-consumers-results.tex <==


% \subsection{Dashboard Consumer Perspectives on Data Trust}
% As participant C04 pointed out that "you can't do generic actions, you have to do specific actions".  Our data-consumer participants are decision makers whose job it is to make tangible, material decisions, not to engage in data analysis for its own sake.  As a result, our interviews found that for decision-making data consumer 1) trust is critical, 2) real-world practicalities sometimes outweigh perfect intellectual comfort, and 3) people fall back on what they know. As we will discuss later, these three findings provide a clear call to action: the data community must innovate and invest in user-accessible tools that increase trust.  Doing so will raise the trust level of day-to-day data-driven decision making, enabling decisions to be made faster and with more confidence.

% \subsection{Data Trust Scenarios}
% The data-trust scenarios described by our data-consumption participants fell into a few general categories. While some scenarios were positive, the majority of scenarios were negative, suggesting that there is room for improvement and innovation in the data-trust space.
% \subsubsection{I trusted the data because I trusted the human producer}
% \begin{displayquote}
% “So I think if we have built a solid relationship with our business partners ... based on honesty, transparency, delivering what we say we will when we say we will,... all those three things kind of equal trust.”[C01]
% \end{displayquote}
% \subsubsection{I trusted the data because I trusted the data pipeline}
% \begin{displayquote}
% “I would say some of it comes down to just day-to-day working in these tools and having them be consistent and not having these kinds of issues I was just describing all the time, having it be in there day in and day out and feeling like it's always a consistent experience to use it and that I see the same things each time.”[C08]
% \end{displayquote}
% \subsubsection{I trusted the data because I had no reason not to}
% \begin{displayquote}
% “So what gives me confidence is the lack of user feedback that something is wrong.”[C10]
% \end{displayquote}

% \subsubsection{The data had been wrong before}
% \subsubsection{Something changed upstream}
% \begin{displayquote}
% "I think another [problem] area is where something changes in an upstream system or something gets categorized in a different way and therefore somehow the values suddenly change, like business logic potentially changes upstream. But it's very hard, the business users don't necessarily tell the people in charge of the data pipes that this changed happened, or they don't realize that this change happened and therefore suddenly the values are weird and you're like 'Oh!', because everything got shoved in a null category as opposed to the category where it was supposed to go because suddenly now things are reclassified."[C10]
% \end{displayquote}
% \subsubsection{Somebody made a mistake or needed training}
% \subsubsection{People weren't aligned on their assumptions}
% \subsubsection{People didn't feel comfortable with their background understanding of the data}
% where data came from
% stats education
% \subsubsection{Insufficient data was presented presented for proper analysis}
% In some instances, it was not the veracity of the data that was called into question but rather the resulting interpretation.  A lack of context rendered the participant unable to properly interpret the data and its significance.
% \begin{displayquote}
% “But I think it's more so that I don't know what I don't know. There is no point of validation. So even if I want to do my own spot checking to go like "Hey, does this look correct?" I've got nothing to validate it against.”[C06]
% \end{displayquote}
% \begin{displayquote}
% “Can you ask the 'compared to what' question? So you've given me three data points for this year. How do those compare with the three data points from the same time period last year? How does this compare to benchmarks and other parts of our industry?”[C09]
% \end{displayquote}

% \subsection{Data Trust Themes}
% All of our participants were part of functional data communities; so, as discussed above, several of the emergent themes were positive in the sense that trust had actually been established.  With that said, accounts of data trust violations inevitably took place in the context of an acute need or problematic situation and as such, some of the themes such as 'Single Source of Truth' or 'Get Your Basics Right' emerged as relatively independent while other themes such as 'Data Smells' and 'Alignment of Assumptions' tended to be more entangled and exhibited a high degree of overlap with other themes.
% \subsubsection{Correctness Matters}
% \subsubsection{Smell, Intuition, and Preference for Human Judgment}
% In the event of a disagreement between data and human recollection, participants generally gave humans the benefit of the doubt.
% \begin{displayquote}
% “[The data say that] [anonymous] did nine engagements and [anonymous] is like, I did 15 engagements. I believe [anonymous] . And in the dashboard if I can't go in and see where that nine came from and do the gap analysis between what [anonymous] said he did and what the dashboard said he did, then I don't trust the dashboard.”[CO2]
% \end{displayquote}
% Even when the data was known to be correct, a person's sensitivity to a data 'smell' was typically given great credence, particularly if that person was a subject matter expert.
% \begin{displayquote}
% "... one [example] was sort of like 'this doesn't smell right'. For a study of [a clinical drug]  we would not expect [these numbers to look like that]."[C08]
% \end{displayquote}
% \textcolor{red}{@nicole, @michael - we should look at other papers regarding people's preference (or lack thereof) for human-generated artifacts and human-controlled AI.}
% \subsubsection{People want recourse if they have questions}
% Participants wanted the ability to follow up on questions.  Sometimes this entailed asking where data came from or how something was calculated, sometimes it entailed learning something new to make sense of the data, and sometimes 
% "So you introduce something new and all of a sudden it's unfamiliar. It's changed. I feel lost and therefore I might push against it or I might not trust it or might not trust you either as a result.”[C09]

% \subsubsection{People want to have access to the low-level data}

% \subsubsection{Single sources of truth are critical}
% A 'single source of truth' was by far the most discussed determinant of data trust.  This notion took on two basic forms: 1) the desire for a single authorized data source and 2) the desire for a single source of definitions and analyses.
% \paragraph{Single Data Source} A single source of data truth was desired when people didn't know which of multiple data sources to use, or which data sources other people were using. 
% \begin{displayquote}
% “The reports that I used to use on [System 1] are now not being up-kept and we're moving to [System 2] reporting. ... I do my forecasting [in System 3]. And then I also look at [System 4]. So there is not one single source of truth or one number that I can depend on.”[C05]
% \end{displayquote}
% Participants also view a single source of data truth as a democratizing and empowering construct that allows any authorized person to consume the data that is being used for decision making.
% \begin{displayquote}
% "And as long as I've connected to that data source, I know the numbers and the data are trustworthy and they're accurate and that was a really kind of empowering thing to be able to do. And you could do that no matter what level you are. You could be an individual contributor who wants to pull some information for a client meeting and it's like 'Cool, I've connected to that, I can trust that.'"[C06]
% \end{displayquote}
% \paragraph{Single Metadata Definition} The specific definitions of concepts like 'territory', 'customer engagement', and 'profit margin' directly impact how those metrics are calculated and thus what numbers are reported. Almost all participants reported that confusion over concept definitions led to misleading data.
% \begin{displayquote}
% "... you've got a room of 10 people you ask, ... how many customers do we have? You'll get 10 different answers. Why? because there's 10 different definitions."[C01]
% \end{displayquote}

% \begin{displayquote}
% "There's just a lot of variation in the way that [finance recognizes revenue].So whenever finance changes the way they do something then it would change how we were able to recognize revenue. And so if that wasn't changed in [our] dashboard then all of a sudden the dashboard is less helpful in determining how successful or unsuccessful we've been, or where the outliers are."[C07]
% \end{displayquote}

% \subsubsection{Communication is important}
% Communication took several forms for our participants, but all agreed that information \textit{about} the data was as important as the data itself. Participant C07 wanted "Something explanatory about the data itself and the calculations" while Participant C08 wanted real time communication about the correctness of the data "because there's crowds of people using this dashboard and we can't afford to have something out there that's giving misinformation."  Relevant to the previous discussion of aligned assumptions, Participant C10 wanted to be told "These are all the different ways that 'engagement' is being calculated". In general, participants were slow to trust data when they didn't know anything about it.


% \subsubsection{When in doubt, go back to basics}
% Decision-making data consumers, while technically savvy people, tended to require that basic analytical foundations be addressed before giving credence to more sophisticated data tools such as forecasting and machine learning.
% \begin{displayquote}
% “But one thing I've noticed is data teams out in the wild, they can get fixated on sort of the really sophisticated kind of predictive kind of experience, but they don't have their descriptive analytics house in order. And so it's almost like they're trying to skip steps and miss the foundations.”[C04]
% \end{displayquote}
% \begin{displayquote}
% "They're like, here we go again, [he’s] got an academic view on this and I'm like, it's actually not an academic view. ...you need at least eight points and then we can talk about it as a trend. It's sort of basic stuff here."[C09]
% \end{displayquote}
% Multiple participants reported that upon first contact with the data or later when an error is perceived they "zoom in and look at the actual data."[C01].  One participant stated “I will always take snapshots of the report that I culled my numbers from."[C05] to have a personal hardcopy should the findings be subsequently called into question.
% %"When something looks bad people want to zoom in and look at the actual data."[C01]
% %“I think the number one thing is I go in the system and I look at the raw data.”[C02]

% %“I will always take snapshots of the report that I culled my numbers from. So then I can link it back to well on this day and this time this is what the report said.”[C05]
